Biexciton State Energies from Many-Body Perturbation Theory Based on Density Functional Theory Simulation

We develop a method for computing self-energy of a biexciton state in a semiconductor nanostructure using many-body perturbation theory (MBPT) based on the density functional theory (DFT) simulation. We compute energies of low-energy biexciton states composed of singlet excitons in the chiral single-wall carbon nanotubes (SWCNT), such as (6,2), (6,5) and (10,5). In all cases we find a small decrease in the biexciton gap: -0.045 $eV$ in (6,2), which is 4.59\% of the non-interacting biexciton gap; -0.041 $eV$ in (6,5), which is 4.47\% of the non-interacting gap and -0.036 $eV$ in (10,5), which is 4.31\%.

==> mypdflatex <==
#/bin/bash

filename=$1
BASENAME=${filename/.*/}

echo $BASENAME
texname="$BASENAME.tex"

normal='\x1b[0m'
highlight='\x1b[31m'
cinfo='\x1b[34m'


#  latex="latex -halt-on-error -interaction=batchmode"
#  latex="latex -interaction=nonstopmode"
#  latex="latex -interaction=errorstopmode"   # haelty an und fragt nach eingabe
#  latex="latex -interaction=batchmode"   # null info
latexfirstrun="pdflatex -halt-on-error -file-line-error -interaction=batchmode"   # null info
latex="pdflatex -halt-on-error -file-line-error -interaction=nonstopmode"   # null info
    # -interaction=STRING     set interaction mode (STRING=batchmode/nonstopmode/scrollmode/errorstopmode)


function compile(){
    $latexfirstrun $BASENAME >/dev/null
    error=$?;
    if [ $error -gt 0 ] ;then
        echo -e "$highlight ############## tex error: $normal"
        $latex $BASENAME |grep -ve '\.pfb>'|grep -ve'^(/usr/share/texmf-texlive/tex/'
        echo -e "$highlight ############## tex error end , stop $normal"
    else
        bibtex $BASENAME >/dev/null     ## for blabla.bib: bibtex blabla
        # bibtex $BASENAME >/dev/null     ## for blabla.bib: bibtex blabla
        $latex $BASENAME >/dev/null
        $latex $BASENAME |grep -ve '\.pfb>'|grep -ve'^(/usr/share/texmf'
        error=$?;
    fi
}
function compileNOBIB(){
    $latexfirstrun $BASENAME >/dev/null
    error=$?;
    if [ $error -gt 0 ] ;then
        echo -e "$highlight ############## tex error: $normal"
        $latex $BASENAME |grep -ve '\.pfb>'|grep -ve'^(/usr/share/texmf'
        echo -e "$highlight ############## tex error end , stop $normal"
    else
#        $latex $BASENAME |grep -ve '\.pfb>'|grep -ve'^(/usr/share/texmf'
#        error=$?;
         echo "ok"
    fi
}




while [ 1 ] ; do
#      fileinfo=$(stat $texname|grep -ie modify);
    fileinfo=$(stat *.tex|grep -ie modify|sort|tail -n1);
    if [ "$fileinfo" != "$oldfileinfo" ] ; then
       compileNOBIB
       echo -e "$cinfo $(date)   : compiled  : $fileinfo   $oldfileinfo $normal"
    fi
    sleep 0.5
    oldfileinfo=$fileinfo;
done

####
remote:

geht ganz gut mit gnome-connect-to-server
ansonsten
sshfs lplolp.dyndns.org:/home/loew/  /home/loew/tmp/lp -o cache_timeout=1
